Estimation of Non-Functional Properties for Embedded Hardware with Application to Image Processing

In recent years, due to a higher demand for portable devices, which provide restricted amounts of processing capacity and battery power, the need for energy and time efficient hard- and software solutions has increased. Preliminary estimations of time and energy consumption can thus be valuable to improve implementations and design decisions. To this end, this paper presents a method to estimate the time and energy consumption of a given software solution, without having to rely on the use of a traditional Cycle Accurate Simulator (CAS). Instead, we propose to utilize a combination of high-level functional simulation with a mechanistic extension to include non-functional properties: Instruction counts from virtual execution are multiplied with corresponding specific energies and times. By evaluating two common image processing algorithms on an FPGA-based CPU, where a mean relative estimation error of 3% is achieved for cacheless systems, we show that this estimation tool can be a valuable aid in the development of embedded processor architectures. The tool allows the developer to reach well-suited design decisions regarding the optimal processor hardware configuration for a given algorithm at an early stage in the design process.

==> gfx/power_time_frag.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{013}[bc][bc]{\matlabtextA Power [W]}%
\psfrag{014}[tc][tc]{\matlabtextA Time [ms]}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $0$}%
\psfrag{001}[ct][ct]{\matlabtextA $1000$}%
\psfrag{002}[ct][ct]{\matlabtextA $2000$}%
\psfrag{003}[ct][ct]{\matlabtextA $3000$}%
\psfrag{004}[ct][ct]{\matlabtextA $4000$}%
\psfrag{005}[ct][ct]{\matlabtextA $5000$}%
\psfrag{006}[ct][ct]{\matlabtextA $6000$}%
\psfrag{007}[ct][ct]{\matlabtextA $7000$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{008}[rc][rc]{\matlabtextA $3.6$}%
\psfrag{009}[rc][rc]{\matlabtextA $3.8$}%
\psfrag{010}[rc][rc]{\matlabtextA $4$}%
\psfrag{011}[rc][rc]{\matlabtextA $4.2$}%
\psfrag{012}[rc][rc]{\matlabtextA $4.4$}%
%
%% </ytick>
